Incrementally Improving Graph WaveNet Performance on Traffic Prediction

We present a series of modifications which improve upon Graph WaveNet's previously state-of-the-art performance on the METR-LA traffic prediction task. The goal of this task is to predict the future speed of traffic at each sensor in a network using the past hour of sensor readings. Graph WaveNet (GWN) is a spatio-temporal graph neural network which interleaves graph convolution to aggregate information from nearby sensors and dilated convolutions to aggregate information from the past. We improve GWN by (1) using better hyperparameters, (2) adding connections that allow larger gradients to flow back to the early convolutional layers, and (3) pretraining on an easier short-term traffic prediction task. These modifications reduce the mean absolute error by .06 on the METR-LA task, nearly equal to GWN's improvement over its predecessor. These improvements generalize to the PEMS-BAY dataset, with similar relative magnitude. We also show that ensembling separate models for short-and long-term predictions further improves performance. Code is available at https://github.com/sshleifer/Graph-WaveNet .

==> proposal.tex <==


\section{Related Work}

\subsection{DCRNN}
The goal of the DCRNN \cite{li2018dcrnn_traffic} paper is to predict traffic at specific locations in a highway network by leveraging both the spatial graph-structure of a connected road network and also recent temporal information at the traffic sensors. The authors use a directed proximity graph and what they call a \textit{diffusion convolution operation} to model the spatial interactions. They then use an RNN (GRU) with seq2seq to model the short-term temporal interactions, outperforming other state-of-the-art algorithms at the time for both the METR-LA and PEMS-BAY datasets.\footnote{We discuss these in greater detail in our proposal section, since we will also use them.} 

\subsubsection{Strengths and Contributions}

There is various literature in this domain that aim to perform node classification in graph structures. 
One novel technical contribution is that the authors model the movement of traffic as a diffusion process on a directed graph, $G$, of the roads. They choose a directed graph because they recognize that roads can be one-way and furthermore that traffic going one direction does not affect traffic going in the opposite direction. They then propose the \textit{diffusion convolution operation}, which combines the data from nearby sensors using a transition matrix for the downstream traffic ($D^{-1}_OW$) as well as the transition matrix for the upstream traffic ($D^{-1}_IW^T$), as shown in equation (2).
%As shown in Equation (2) they aggregate neighborhood information with learned weights, so that if traffic is backed up near a sensor it will predict higher subsequent traffic for the affected nearby sensors.

\includegraphics[width=13cm]{dcrnn_equation.png}
\\Equation 2: the $\theta$ parameters are learned conv filters, $D^{-1}_OW$ and $D^{-1}_IW^T$ are the downstream and upstream transition matrices respectively, $X$ is the feature vector from the traffic sensors, and $P$ is the number of features at each node.

An additional technical contribution is the authors' application of a GRU to the traffic data. They treat traffic much like a seq2seq machine translation problem (backprop through time, etc.). They introduce DCGRU, which stands for Diffusion Convolution Gated Recurrent Unit, which is like the standard GRU unit except all the matrix multiplications in the GRU gate equations are replaced with (parameterized) diffusion convolutions. They also introduce what they call "scheduled sampling": they gradually increase the continuity between the encoder and decoder throughout training, starting with feeding only ground truth to the decoder and eventually only feeding the encoder's output to the decoder, as occurs at test time.

The DCRNN paper combines graph features (road proximity) with non-graph features (velocity, volume, and other sensor readings) and uses machine learning to make predictions about the nodes, one of the primary objectives of this class. One strength of the paper is how thorough it is with ablation studies. Given the complexity of the approach, there were many times when a reader might ask whether all of these steps were necessary.
\subsubsection{Critique and Future Work}

One weakness of the paper is that, although the authors call their spatial approach convolutional, they do not re-use filters in a sliding window approach, as traditional convolutional networks do. Doing so may decrease the complexity of the operation and number of parameters the graph has to learn. It also may decrease performance, but seems like an experiment worth doing and a discrepancy in terminology worth acknowledging. Another weakness of the paper is simply how complex the approach is. This aspect of the paper is improved upon by the next paper in our related work section, Graph Wavenet. %We didn't find any assumptions or design choices particularly unrealistic in this paper.

Two areas that the paper specifies for future work are applying the proposed model to other spatio-temporal forecasting tasks and extending to the case where the underlying graph structure is changing in time, like detours caused by construction. One interesting direction to take this paper might be to apply their approach to weather data or neuroscience, but that would require some data curation and thus seems unwise for a class project.

% Maybe we should move this to proposal, I asked on Piazza.
Given that Graph WaveNet was published after this paper and outperformed it, we are very interested in investigating different architectural approaches further. Another temporal field that used to be modeled mostly by recurrent neural networks is that of natural language processing. In the last couple of years, however, most natural language processing tasks have performed much better when using transformer networks than recurrent networks. We are therefore interested in how well transformers with self-attention could model the spatial and temporal traffic data. We might also try to apply a convolutional approach that uses a sliding window and therefore applies the same filters to each neighborhood of nodes as another architecture investigation.

If the transformer direction seems to be a dead end, there is a lot of interesting anaylsis work we could do. The authors investigate filter weights as a sanity check that traffic sensors closest to the location of interest are weighted most heavily, but they do not dive deeply into where this method performs best/worst and why. An extensive error analysis could be very enlightening and highlight missing features or inspire architecture changes for the future.
\subsection{Graph Wavenet}
Using identical data and evaluation metrics, \citet{gwn} slightly improve over DCRNN in the key METR-LA metric, predicting traffic 1 hour ahead, but, more notably, reduce training time by a factor of 6 and inference time by a factor of 10. These speedups are accomplished by switching timeseries processing from a sequential RNN backbone to a 1D dilated convolution backbone, inspired by the Wavenet architecture first proposed by \citet{wavenet}  for audio generation.

\subsubsection{Strengths}
Overall, the assumptions and design choices in this paper made sense to us. One key strength of this paper is the use of convolution. Whereas RNN's process sequentially and update a hidden state, convolutional architectures, as well as transformers, process sequences all at once, making forward and backward passes parallelizable on GPUs.

The receptive field size of stacked dilated casual convolution networks grows exponentially with an increase in the number of hidden layers, as shown in Figure 2, where the receptive field of the top ($k=3$) layer is 8 timesteps (40 minutes). 

Another key strength of the paper is the use of a flipped version of the adjacency matrix, (DCRNN also does this), which encodes road network strength. Even if there is no direct dependency between traffic ahead and traffic behind, accidents in front of fast moving traffic can propagate the slow down to previous sensors that only have out-edges to the sensor at the site of the crash. The authors show that much of their performance gain is from using this extra information, but do not show an ablation where they only use the backward adjacency matrix, which could answer whether most traffic is from accidents (backwards) or passengers leaving work/home at the same time (forwards).

The authors also note that the weighted adjacency matrix provided with the data is not perfect: some nodes that are not connected affect each other, and some nodes that don't affect each other are connected. They propose learning an "adaptive" adjacency matrix from the data, and update its weights with backpropagation. They claim that this also allows their method to work in situations where no adjacency matrix is provided, and run ablation studies showing only slightly degraded performance when only the adapative adjacency matrix is used. Once forward and backward adjacency matrices are used, however, the added contribution of also using the adaptive matrix is very small.
%In the reference code, the adaptive adjacency matrix's parameters are initialized from an SVD decomposition of the true adjacency matrix -- so the experiment result does not justify the claim of relaxed data requirements. 
% ^^ controlled by `aptinit` param, not obviously turned on?
\subsubsection{Weaknesses}
\textbf{Skip Connections Discard Information} Each layer downsamples the time dimension of the tensor by 1 or 2, so skip connections of previous layers discard the outputs for the "extra timesteps" from the earliest part of the previous output. ("Skip Connections" in architecture diagram). 

Similarly, the "residual" connection that goes around the Gated TCN block's output is too large, and is truncated to match the GCN's output in size.

In both cases, it might work better to mean or max pool instead of throwing away information, or use padded convolutions to keep tensors the correct shape.

\textbf{Missing Ablations}
In the architecture diagram, TCN-a and TCN-B and are both 1x1 convolutions with the same input channels, output channels and dilation. The only difference is the activation functions before the elementwise multiplication. It would be interesting to know whether these similar modules improve performance, or are learning different things.
Similarly, it would be interesting to know how much history is useful for traffic prediction. Does the model effectively utilize more history than RNN based models?

Finally, the authors do not consider block designs that aggregate neighborhood information before processing timeseries--flipping the order of the GCN and Gated TCN blocks in the architecture diagram, for example.

% Finally, the authors' Table 5 shows that without the adaptive adjacency matrix, their method significantly underperforms DCRNN. This motivates continued use of the adaptive adjacency matrix for graph convolution, but experiments that test whether the dilated convolution system for timeseries processing can be improved upon, either by RNN or recently popularized transformers.

\textbf{Using full graph each forward pass:}
Each input tensor is shaped (batch size, $F$, $|V|$, $|T|$), which might prevent using this approach on graphs that are larger than 207 nodes.  Additionally, multiple copies of the full adjacency matrix, and their gradients, are stored in GPU memory each iteration. Using the sparsity of the adjacency matrix could help alleviate this issue.
\begin{center}
    \includegraphics[scale=0.3]{dilation_receptive_field.png}
\end{center}
% Adaptive Adjacency Matrix
%and improves 6x in training time by eliminating Backprop through time and replacing the GRU logic with dilated convolution, which slides over inputs, but skips values. Their figure explains it a bit better:
%In this figure the top layer would have receptive field size 8. The authors set the receptive field to have the same size as the input sequence length.
%"true" adjacency matrix and this dependency must be learned.
%I don’t really understand where the authors’ learned “adaptive dependency matrix.”, but apparently it eliminates some data issues: The math doesn’t look very much like attention computations, so this might be an opportunity for improvement!
\subsection{Graph Attention Networks}

At a high level, the “Graph Attention Network” (\cite{graph_attn_networks}) paper proposes a new method for classifying nodes of a graph using graph attention networks, which leverage masked self-attention layers to address the shortcomings of prior graph convolution based work. More concretely, this network involves stacking layers to attend over the features of neighboring nodes in order to implicitly weight them, thereby learning the hidden representation of each node in the graph in a computationally inexpensive manner. The proposed method is suitable for both the \textit{transductive} (same test graph) and \textit{inductive} (new test graph) flavors of semi-supervised problems. It was evaluated on the CORA, Citeseer and Pubmed citation network benchmarks and protein-protein interaction dataset and achieved or surpassed state-of-the-art results, making a case for attention-based models to deal with arbitrarily structured graphs. The goal of the paper, node classification, aligns well with the topics presented in the course.

\subsubsection{Strengths}
One strength of the proposed network is its overall efficiency, both from a computational and storage standpoint. Specifically, the computation of attentional coefficients can be parallelized across all edges of the graph and similarly the aggregation can be parallelized across all nodes, without requiring complex matrix operations or spectral operations. In fact, the GAT layer can be implemented with only sparse matrix operations, reducing storage to merely $O(V + E)$, making it more feasible for large graphs. %This benefit becomes particularly important as we try to study very large graph networks.
\begin{center}
\includegraphics[scale=0.3]{gat.png}    
\end{center}
Another strength of this paper is the unique combination of attention and local graph representation learning (Figure 1). The use of the masked attention mechanism is clever as it provides a mechanism to infer structural information of the graph (since the attention coefficients are calculated for the neighbors in the egonet of a node), without requiring knowledge of the entire global graph structure. This shared edge-based mechanism not only offers increased scalability but also offers the ability for graph-attention networks to work on test graph structures that were never trained on before. In the context of this problem, the use of multi-head attention--where operations are replicated and the outputs are accumulated feature wise--is noteworthy.  This not only allows for controlling the learning process of the model (a good regularization technique) but also jointly attending information from different vantage points, wherein each head effectively offers a different “importance” for the nodes around a specific focal point. All in all, we didn't find any assumptions or design choices particularly unrealistic in this paper.

\subsubsection{Weaknesses/ Future Exploration}
One weakness of this paper is the authors’ neglect for exploring whether learning information past merely the local neighbors (at a 1-hop distance) would improve accuracy or at least mentioning why they believed non-local information would not help in classifying a specific node of a network. Some algorithms we have explored in this class, for instance the structural algorithm ReFeX, explicitly try to aggregate features recursively from neighbors of neighbors to obtain an understanding of the structure at a slightly higher level. It seems like in many cases, it would be beneficial to exploit the larger graph structure rather than simply the first order neighbors, so this is one area of exploration we could consider.  This gives rise to potential project extensions such as exploring skip connections or neighborhood aggregation with directional biases (focusing on certain neighbors over another because they are more important).

In addition, one aspect that this paper mentioned only briefly and could have explored further is whether performance could be improved by removing redundant computation. Specifically, during the parallelized computation process across edges, since neighborhoods of various neighbors overlap significantly, there is an opportunity to avoid computing the same thing twice. This is a viable project exploration aspect as well-- see whether we can “cache” the result of repeated work and use dynamic programming to further improve the efficiency of the model.

A final critique of this paper is the lack of diversity in the experiments. First of all, it focused primarily on citation network benchmarks and did not show much generalizability. Accordingly, one area we could explore is how this model does on other networks, for instance traffic data or social network data. Additionally, the paper lacks graphs on hyperparameter selection and fails to provide intuition as to why specific design choices were made.  For example, doing a parameter sweep on the number of attention heads or the dropout percentage would solidify the overall decision process.

\section{Proposal}
\subsection{Problem/Hypothesis}
Transformer architectures have led to significant improvements over Convolutional architectures in the processing of natural language sequences. Additionally, \citet{graph_attn_networks} show that that attention mechanisms can improve node classification performance on static or changing graphs. We aim to examine whether these attention mechanisms can be used to improve traffic prediction.

This work is motivated by the success of Graph Wavenet's architectural improvements, but the lack of large benefit that work derived from it's parametrized adjacency matrix. We suspect that deeper more advanced forms of attention might deliver larger benefits.

\subsection{Data}
We use the same traffic datasets as two of the papers in our Related Works section: 

\includegraphics[scale=0.3]{data_desc.png} 

\textbf{METR-LA} This dataset comes from loop detectors in the highway of Los Angeles County. These detectors collect features such as velocity and volume over time. We use 4 months of data and 207 sensors, the same as the DCRNN and GWN papers.

\textbf{PEMS-BAY} This dataset is similar to METR-LA but collected by California Transportation Agencies (CalTrans) Performance Measurement System (PeMS) in the Bay Area. We use the same 325 sensors and 6 months of data as the DCRNN and GWN papers.

In these datasets, the directed adjacency matrix  (provided by the DCRNN authors) is based on the driving distance from one sensor to another in meters. This means that nearby sensors have large weights, but also means that sensors in zones with much less traffic are considered to have strong connections to zones that have less traffic, even if they don't have enough traffic to actually influence the next sensor. Attention mechanisms might learn to ignore these unimportant neighbors.

\textbf{Measurement:} We will use the same ``MAPE @12" metric as Graph Wavenet (GWN) and DCRNN. This measures the average percentage error of predicted traffic 1 hour ahead. GWN's state of the art result is 2.53\%.

\subsection{Method/Execution}
Since we do not know which experiments will work, we propose a series of experiments in order of difficulty so that if an experiment succeeds we can investigate it further, and if it fails we can move down the list. We will measure the success of each experiment using the mean average percentage error predicting traffic one hour ahead, called ``MAPE @12". We will also analyze existing models' errors in parallel with experimentation, in order to generate more experiment ideas.\\
\newline \textbf{Experimental Agenda:}
\begin{enumerate}
    \item Replace GWN's Gated TCN block with a small transformer.
    \item Add transformers to the Graph Convolution block of GWN.
    \item GWN Block Design Weakness: aggregate neighborhood information before timeseries processing. 
    \item Use pooling or padding to address the "Skip Connections Discard Information" issue with GWN discussed earlier.
\end{enumerate}

We would also like to measure how much history other approaches are considering. While the graph wavenet paper shows that 1-D conv can cover 12 timesteps back, it might be desirable to use more than an hour of history for some cases, or directly use information about what happened 24 hours ago in the model.\\\\
Capturing the kind of errors the models makes help gain insight into how well our proposed solution works. For example, we would love to know whether the  existing models ignore seasonality and whether connection strengths depend on time of day/day of week. Given we
have various experiment ideas and associated fallback plans, overall we believe the project seems feasible, while being technically challenging and providing us opportunities to learn and contribute to graph networks research.
